Short-term forecasting of Amazon rainforest fires based on ensemble decomposition model

Accurate forecasting is important for decision-makers. Recently, the Amazon rainforest is reaching record levels of the number of fires, a situation that concerns both climate and public health problems. Obtaining the desired forecasting accuracy becomes difficult and challenging. In this paper were developed a novel heterogeneous decomposition-ensemble model by using Seasonal and Trend decomposition based on Loess in combination with algorithms for short-term load forecasting multi-month-ahead, to explore temporal patterns of Amazon rainforest fires in Brazil. The results demonstrate the proposed decomposition-ensemble models can provide more accurate forecasting evaluated by performance measures. Diebold-Mariano statistical test showed the proposed models are better than other compared models, but it is statistically equal to one of them.

==> Body/MaterialAndMethods.tex <==
\section{Material \label{MAM}}

% \begin{wrapfigure}{R}{0.5\textwidth}
%   \vspace{-20pt}
%   \begin{center}
%     \includegraphics[width=0.48\textwidth]{Figures/amazon-map}
%   \end{center}
%   \vspace{-20pt}
%   \caption{Brazilian Amazon rainforest area\label{fig:map}}
%   \vspace{-10pt}
% \end{wrapfigure}
The dataset analyzed in this paper refers to active fire spots in Brazilian Amazon rainforest area 
% (see illustration in Figure~\ref{fig:map}) 
collected from the database of Fire Program of the Brazil's National Institute for Space Research (INPE) \cite{INPE2019}. 
% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width = 0.5\textwidth]{Figures/amazon-map.png}
%     \caption{Brazilian Amazon rainforest area\label{fig:map}}
% \end{figure}
The dataset consists in 255 observations monthly since June 1998 to August 2019. To determine system lags to create inputs, simulations was conducted varying the lag from 1 to 10, which lag equals to 10 (where the training data started since April 1999) presented better results. Moreover, the dataset was splitted into training and test sets in proportion of 70\% and 30\%, respectively. In Table~\ref{tab:summary} is presented a summary of the statistical indicators of the dataset, which are the Maximum (Max), Minimum (Min), Mean and Standard Deviation (Std).

\begin{table}[!htb]
\scriptsize
\centering
\begin{tabular}{llccccc}
\hline
Variable                        & Samples                     & \# of     & \multicolumn{4}{c}{Statistical indicator}   \\ \cline{4-7}
                                &                             & Samples   & Max       & Min      & Mean      & Std      \\ 
\hline
Fire spots                      & All set                     & 245       & 73141     & 70       & 9427      & 13249.01 \\
                                & Training set                & 171       & 73141     & 70       & 10273     & 14788.60 \\
                                & Test set                    & 74        & 36569     & 379      & 7473      & 8477.56  \\
\hline
\end{tabular}
\caption{Summary of the statistical indicators of the dataset\label{tab:summary}}
\end{table}


% \subsection{Seasonal and Trend Decomposition Using Loess}

% The subdivision of the forecasting problem into smaller parts is achieved through a decomposition procedure which disaggregates the global series into three additive components, namely the trend, seasonality and error. The seasonal and trend decomposition using Loess (STL), presented by \cite{cleveland1990stl} is versatile and robust to decompose time series. STL performs additive decomposition of the data through a sequence of applications of the Loess smoother, applying locally weighted polynomial regressions at each point in data set. Furthermore, STL can handle any type of seasonality, as well as, the flexibility to change not only the seasonal component over time, but also to control the rate of change. The most important advantages of the STL, relative to other decomposition techniques, is its strong robustness to outliers in the data and ease of use \cite{xiong2018seasonal}. The decomposition is calculated as, 

% \begin{equation}
% y_{t}=S_{t}+T_{t}+R_{t}, 
% \end{equation}
% where $y_t$ is the time series at time $t$, the $S_t$, $T_t$ and $R_t$, refers to the seasonal, trend and remainder components, respectively.

% \subsection{Multivariate Adaptive Regression Splines Method}

% Multivariate adaptive regression splines (MARS) is a nonlinear and nonparametric regression and classification approach proposed by \cite{friedman1991multivariate}. It is a method to predict the values of a continuous dependent variable from a set of predictors. It is flexible for high dimensional data motivated by a recursive partitioning approach to regression \cite{sekharroy2018estimating}. MARS defines the functional relation between the dependent and independent variables by means of a group of coefficients and piecewise polynomials, called splines (basis functions). The MARS model has the capability of finding optimal variable transformations, interactions and complex data which are often hidden in high-dimensional data dependencies. The MARS regression model fits the base functions to different intervals of the independent variables. MARS can be defined as

% \begin{equation}
% \hat{y}=\hat{f}(x)=\beta_{0}+\sum_{n=1}^{N} \beta_{n} g_{n}(x),
% \end{equation}
% where $\hat{y}$ denotes the prediction value of output variables, $\beta = \{\beta_{O}, \ldots, \beta_{n}\}$ denotes weight parameter of the basis function, $g_n(x)$ denotes the $n$th basis function.

% \subsection{Support Vector Regression}

% Support Vector Regression (SVR) was introduced by \cite{cortes1995support} to solve classification tasks and then was extended to solve regression problems  \cite{Drucker1997}. The main idea behind this methodology consists in determining points close to a hyperplane, support vectors, that maximize the margin between two classes obtained from the difference between the target value and a threshold \cite{ribeirong2019ensemble}. Several kernels functions are stated in the literature, and in this paper the Radial Basis function (RBF) employed in developing the SVR model in this study, can be expressed as: 

% \begin{equation}
%     K\left(\mathbf{x}, \mathbf{x}^{\prime}\right)=\exp \left(-\frac{\left\|\mathbf{x}-\mathbf{x}^{\prime}\right\|^{2}}{2 \sigma^{2}}\right),
% \end{equation}
% where $\left\|\mathbf{x}-\mathbf{x}^{\prime}\right\|^{2}$ may be recognized as the squared Euclidean distance between the two feature vectors, and $\sigma$ is a parameter \cite{vert2004primer}.

% \subsection{Boosted Generalized Linear Model}

% Boosted Generalized Linear Model (GLMBoost) is a generalized linear model (GLM) based on a component-wise gradient Boosting \cite{breiman1998} firstly proposed by \cite{buhlmann2003boosting}. This model can be essentially interpreted in the same way which models derived from GLM, however, GLMBoost additionally performs variables selection and the effects are shrunken toward zero if early stopping is applied. The GLM can be  stated by a linear predictor $\eta_{i}=\beta_{0}+\beta_{1} x_{1 i}+\ldots+\beta_{p} x_{p i}$, where $\beta$ is a unknown coefficient; a link function $g\left(\mu_{i}\right)=\eta_{i}$, that describes how the mean, $E\left(Y_{i}\right)=\mu_{i}$, depends on the linear prediction; and a variance function $\operatorname{var}\left(Y_{i}\right)=\phi V(\mu)$ that describes how the variance, $\operatorname{var}\left(Y_{i}\right)$ depends on the mean, where the dispersion parameter $\phi$ is a constant.



